UAVs with Reconfigurable Intelligent Surfaces: Applications, Challenges, and Opportunities

A reconfigurable intelligent surface (RIS) is a metamaterial that can be integrated into walls and influence the propagation of electromagnetic waves. This, typically passive radio frequency (RF) technology is emerging for indoor and outdoor use with the potential of making wireless communications more reliable in increasingly challenging radio environments. This paper goes one step further and introduces mobile RIS, specifically, RIS carried by unmanned aerial vehicles (UAVs) to support cellular communications networks and services of the future. We elaborate on several use cases, challenges, and future research opportunities for designing and optimizing wireless systems at low cost and with low energy footprint.

==> include/contribution.tex <==

The      



==> include/otherUAVservices.tex <==

\begin{table*}[ht]
\centering
\caption{KPIs for UAV-assisted wireless services~\cite{UAS_5G}}

{\begin{tabular}{|p{3.4cm}|p{2.7cm}|p{1.3cm}|p{1.6cm}|p{1.4cm}|p{1.3cm}|p{3.2cm}|}
\hline
\centering
\textbf{Services} & \textbf{Uplink \newline Data rate} & \textbf{Uplink Latency} &\textbf{Downlink Data rate} & \textbf{Downlink Latency} & \textbf{Height} &  \textbf{service area}
\\ \hline
\vspace{-0.05 in}
8K video live broadcast &
\vspace{-0.05 in}
100 Mbps
&
\vspace{-0.05 in}
200 ms
&
\vspace{-0.05 in}
600 Kbps
&
\vspace{-0.05 in}
20 ms
&
\vspace{-0.05 in}
$<$ \text{100 m}
&
\vspace{-0.05 in}
Urban, scenic area
\\ \hline
\vspace{-0.05 in}
{4*4K AI surveillance} &
\vspace{-0.05 in}
120 Mbps
&
\vspace{-0.05 in}
20 ms
&
\vspace{-0.05 in}
50 Mbps
&
\vspace{-0.05 in}
20 ms
&
\vspace{-0.05 in}
$<$ \text{200 m}
&
\vspace{-0.05 in}
Urban, rural area
\\ \hline
\vspace{-0.05 in}
{Remote UAV controller through HD video} &
\vspace{-0.05 in}
\geq \text{25 Mbps}
&
\vspace{-0.05 in}
100 ms
&
\vspace{-0.05 in}
300 Kbps
&
\vspace{-0.05 in}
20 ms
&
\vspace{-0.05 in}
$<$ \text{300 m}
&
\vspace{-0.05 in}
Urban, rural area
\\ \hline
\vspace{-0.05 in}
{Real-Time Video} &
\vspace{-0.05 in}
0.06 Mbps 
&
\vspace{-0.05 in}
100 ms
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
Urban, rural, countryside
\\ \hline
\vspace{-0.05 in}
{Video streaming} &
\vspace{-0.05 in}
4 Mbps\to  \text{720p } \newline\text{video} \newline
9\text{ Mbps}\to \text{1080p } \newline\text{video}  
&
\vspace{-0.05 in}
100 ms
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
Urban, rural, countryside
\\ \hline
\vspace{-0.05 in}
{Periodic still photos} &
\vspace{-0.05 in}
1 Mbps
&
\vspace{-0.05 in}
1 s
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
\centering
-
&
\vspace{-0.05 in}
$<$ \text{120 m}
&
\vspace{-0.05 in}
Urban, rural, countryside
\\ \hline
\end{tabular}%
}
\label{tab:KPI1}
\end{table*}
